Reactive Navigation in Partially Familiar Planar Environments Using Semantic Perceptual Feedback

This paper solves the planar navigation problem by recourse to an online reactive scheme that exploits recent advances in SLAM and visual object recognition to recast prior geometric knowledge in terms of an offline catalogue of familiar objects. The resulting vector field planner guarantees convergence to an arbitrarily specified goal, avoiding collisions along the way with fixed but arbitrarily placed instances from the catalogue as well as completely unknown fixed obstacles so long as they are strongly convex and well separated. We illustrate the generic robustness properties of such deterministic reactive planners as well as the relatively modest computational cost of this algorithm by supplementing an extensive numerical study with physical implementation on both a wheeled and legged platform in different settings.

==> Makefile <==
#
#  Makefile for automating LaTeX related tasks and administrating a 
#  directory of numerous thesis-related files.
#
#  Prepared by Neil C. Miller
#  Modifed by Lord Simon Cuce III
#  May, 1997
#
#  Revision 2.0 5/12/97
#

INCLUDEFILES = 

	FILENAME = body
	ARCHIVE = backup
	PAPERTYPE = a4

.DEFAULT:
	@echo Sorry, that is an undefined target.

help:
	@echo
	@echo Help for make utility:
	@echo
	@echo   make	    - shows this help.
	@echo   make dvi	- executes latex one time.
	@echo   make clean      - removes all backup and output files.
	@echo   make ps	 - executes dvips one time.
	@echo   make bib	- executes bibtex one time.
	@echo   make all	- runs latex several times, bibtex and dvips.
	@echo   make backup     - creates a .tar.gz backup of all files.
	@echo
	@echo Filenames for the main document and backup archive are 
	@echo specified in the Makefile.
	@echo

%:	
	@echo "$@" | latex $(FILENAME) 

dvi:
	@echo $(INCLUDEFILES)  | latex $(FILENAME)

clean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps

realclean:
	@$(RM) *% *.bak *.dvi $(FILENAME).ps *.aux *.bbl *.blg *.ilg *.ind *.lof *.log *.lot *.lof *.toc *.loa *~

ps:
	@dvips -G0 -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)
goodps:
	@dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o $(FILENAME).ps $(FILENAME)

pdf:
	dvips -G0 -Ppdf -R0 -t$(PAPERTYPE) -o tmp.ps $(FILENAME)
	ps2pdf -dCompatibilityLevel=1.4 -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=$(PAPERTYPE) tmp.ps $(FILENAME).pdf
	$(RM) -f tmp.ps

bib:
	@bibtex $(FILENAME)

# This doesn't work perfectly.  For example, the changing of a section
# name does not cause a Warning, even though its change will not be 
# reflected in the TOC until the next pass.  So, "all" should be done 
# after "realclean" before final submission.  Possibly a good use for a 
# small perl script which checks to see that the TOC is up-to-date.
all:
	echo '** Running LaTeX **'
	echo $(INCLUDEFILES) | latex $(FILENAME);
	@if ( grep "There were undefined references"        \
			$(FILENAME).log >/dev/null ); then  \
		echo '** Running BibTeX **';                \
		bibtex $(FILENAME);                         \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	fi
	@while ( grep "Rerun to get cross-references"       \
			$(FILENAME).log >/dev/null ); do    \
		echo '** Re-running LaTeX **';              \
		echo $(INCLUDEFILES) | latex $(FILENAME);  \
	done

oldall:
	@latex $(FILENAME)
	@bibtex $(FILENAME)
	@latex $(FILENAME)
	@latex $(FILENAME)

allps: all
	@dvips -G0 -Ppdf -o $(FILENAME).ps $(FILENAME)

backup:
	@$(RM) $(ARCHIVE).tar.gz
	@tar cf $(ARCHIVE).tar *
	@gzip $(ARCHIVE).tar
	@ls -l $(ARCHIVE).tar.gz

